REA: A Routed Embodied Agent Runtime for Asynchronous Brain-Cerebellum Control

Foundation models are becoming remarkably reliable at high-level reasoning, yet they remain too slow and costly to serve as fine-grained controllers. Conversely, fast policies like VLAs and whole-body controllers offer more efficient reflexes, but struggle to generalize. While pairing a deliberative brain (foundation models) with a reactive cerebellum (fast policies) seems natural for embodied systems, two obstacles remain: methods are built and scored on incompatible stacks, and their asynchronous coordination is difficult. For example, an agent that calls the VLA in the agentic loop can stall the fast execution, while a VLA that calls the agent on errors tends to re-trigger fallbacks repeatedly or completely miss silent failures. To address this, we propose REA (Routed Embodied Agent), a unified runtime where a deliberative System 2, an embodied router System 1 and reactive System 0 policies cooperate under a single golden rule - no running policy waits on the brain. Instead of querying the brain at each failure, REA employs a route memory that stores each policy's measured success ahead of time, a boundary-triggered judge gate that consults the brain on policy execution, and a shared-budget escalation ladder for bounded recovery. Evaluated on 3,000 test episodes across 60 LIBERO-Pro tasks, REA reaches 95.9% success and beats the best single-agent baseline in its own policy pool (94.7%) while reducing control steps by 25% and control time by 17%. In a separate 100-episode RoboTwin 2.0 study, REA achieves 84% success with VLA policies and 86% with VLA+code, compared with 80% for the strongest single VLA baseline MEDex. These results demonstrate learned and programmatic policies operating within the same runtime. REA also transfers to BEHAVIOR-1K and a real Unitree G1 humanoid, achieving the highest observed success among the compared methods.

==> abstract.tex <==
\begin{abstract}
Foundation models reason well but remain too slow and costly for fine-grained control, while fast policies often struggle to generalize. Combining them is difficult because existing systems use incompatible execution and evaluation stacks, and poorly timed brain calls interrupt control or miss silent failures. We present REA (Routed Embodied Agent), a three-level runtime comprising a deliberative System 2, an embodied router System 1 and reactive System 0 policies. Route memory selects policies using development results, a boundary-triggered judge checks completion after a policy returns, and an escalation ladder supports recovery under a shared budget. No running policy waits for the brain. On 3,000 test episodes across 60 LIBERO-Pro tasks, REA achieves 95.9\% success versus 94.7\% for the strongest individual baseline in its policy pool, with 25\% fewer control steps and 17\% less control time. Where policies fail silently, judge gating adds 3.1\% over exception handling at 2.1$\times$ the time per success. In a separate 100-episode RoboTwin~2.0 study, REA achieves 84\% success with VLA policies and 86\% with VLA+code, compared with 80\% for MEDex, the strongest single VLA baseline. These results demonstrate learned and programmatic policies operating within the same runtime. REA also transfers to BEHAVIOR-1K and a real Unitree G1 humanoid, achieving the highest observed success among the compared methods.
\end{abstract}

